An Efficient Implementation of Guard-Based Synchronization for an Object-Oriented Programming Language

In the shared variable model of concurrency, guarded atomic actions restrict the possible interference between processes by regions of atomic execution. The guard specifies the condition for entering an atomic region. That is a convenient model for the specification and verification of concurrent programs, but has eschewed efficient execution so far. This article shows how guarded atomic actions, when attached to objects, can be implemented highly efficiently using a combination of coroutines, operating-system worker threads, and dedicated management of object queues and stacks. The efficiency of an experimental language, Lime, is shown to compare favourably with that of C/Pthreads, Go, Erlang, Java, and Haskell on synthetic benchmarks.

==> eptcsdata.tex <==
\providecommand{\firstpage}{44}
\providecommand{\publicationstatus}{Farzaneh Derakhshan \& Jan Hoffmann (Eds.): 16th International\\ Workshop on
Programming Language Approaches to Concurrency\\
and Communication-cEntric Software 2025 (PLACES 2025)\\
EPTCS 420, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.420.5}{10.4204/EPTCS.420.5}}
\pdfoutput=1

